Distance-Guided GA-Based Approach to Distributed Data-Intensive Web Service Composition

Distributed computing which uses Web services as fundamental elements, enables high-speed development of software applications through composing many interoperating, distributed, re-usable, and autonomous services. As a fundamental challenge for service developers, service composition must fulfil functional requirements and optimise Quality of Service (QoS) attributes, simultaneously. On the other hand, huge amounts of data have been created by advances in technologies, which may be exchanged between services. Data-intensive Web services are of great interest to implement data-intensive processes. However, current approaches to Web service composition have omitted either the effect of data, or the distribution of services. Evolutionary Computing (EC) techniques allow for the creation of compositions that meet all the above factors. In this paper, we will develop Genetic Algorithm (GA)-based approach for solving the problem of distributed data-intensive Web service composition (DWSC). In particular, we will introduce two new heuristics, i.e. Longest Common Subsequence(LCS) distance of services, in designing crossover operators. Additionally, a new local search technique incorporating distance of services will be proposed.

==> document.tex <==
In discrete combinatorial optimization research, Cowling et
al. [11] coined the term “hyperheuristic” to describe the idea
of fusing a number of different memes together, so that the actual
meme applied may differ at each decision point, i.e., often
at the chromosome/individual level. They describe the hyperheuristic
as a heuristic to choose memes. The idea of using multimemes
and adaptive choice of memes at each decision point
was also proposed by Krasnogor et al. in [13], [14]. At about
the same time, Smith also introduced the co-evolution of multiple
memes in [15], [20]. 
From our survey1, it is noted there has been a lack of studies
analyzing and comparing different adaptive MAs from the perspective
of choosing memes. 

“meta-Lamarckian learning”, “hyperheuristic”,
and “multimemes”

In the context of combinatorial optimization, Cowling et al. [11] introduced the term
“hyperheuristic” as a strategy that manages the choice of which
meme should be applied at any given time, depending upon
the characteristics of the memes and the region of the solution
space currently under exploration. 

The choice function proposed in [11], [12] is composed of three
components. The first component represented by reflects the
recent improvement made by a meme and expresses the idea that
if a meme has recently performed well, it is likely to continue to
be effective. The second component describes the improvement
contributed by the consecutive pairs of memes, and the
last component records the period elapsed since a meme was
last used. 

2) Multimemes and Co-Evolving MAs: Krasnogor also
proposed a simple inheritance mechanism for discrete combinatorial
search [13], [14]. Each individual is represented and
composed by its genetic material and memetic material. 
